Loss- and Reward-Weighting for Efficient Distributed Reinforcement Learning

This paper introduces two learning schemes for distributed agents in Reinforcement Learning (RL) environments, namely Reward-Weighted (R-Weighted) and Loss-Weighted (L-Weighted) gradient merger. The R/L weighted methods replace standard practices for training multiple agents, such as summing or averaging the gradients. The core of our methods is to scale the gradient of each actor based on how high the reward (for R-Weighted) or the loss (for L-Weighted) is compared to the other actors. During training, each agent operates in differently initialized versions of the same environment, which gives different gradients from different actors. In essence, the R-Weights and L-Weights of each agent inform the other agents of its potential, which again reports which environment should be prioritized for learning. This approach of distributed learning is possible because environments that yield higher rewards, or low losses, have more critical information than environments that yield lower rewards or higher losses. We empirically demonstrate that the R-Weighted methods work superior to the state-of-the-art in multiple RL environments.

==> Sections/Discussion.tex <==
\section{Discussion}
%Methods
\subsection{Reward weighted}
Weighting based on reward -> higher rewards have a larger impact, should lead to actions which give higher rewards
Would also mean that the predictions for lower reward actions are more likely to not be as good, even if the episodes should include quite a lot of these actions anyways.

\subsection{Loss Weighted}
Weighting based on loss -> Higher loss means reward predictions are worse, so should lead to faster learning
Though it is already accounted for in the calculation of the loss, given that the weight is lower than 1 it should not matter.
This is similar to the reward in that the sum of the weights should not exceed the number of agents.
If this is done, the gradients could overstep significantly.

\subsection{Actors gradient plus average gradient}
Using the gradient of the actor and adding the average gradient of all actors, given that they start in the same location -> the actors spread from the initial location in the gradient, which could lead to a faster global optimum.
The issue is that it may also lead to the actors gradients spreading too much, which would lead to the updates not optimizing the individual agents gradients at all.

\subsection{Actors gradient plus sum gradient}
Using the gradient of the actor and adding the average gradient of all actors, given that they start in the same location -> the actors spread from the initial location in the gradient, which could lead to a faster global optimum.
The issue is that it may also lead to the actors gradients spreading too much, it is more likely to make each actor stay close as the gradient updates will include more of the other actors gradient, but it could lead to the updates not optimizing the individual agents gradients at all.

\subsection{Weighted hyperparameters}
Both Loss and Reward weighted updates included a hyperparameter, this simply added a small number to the weight, so that no agent is forgotten even if their loss is too low, or their reward is too low.
There is something to learn from any update done by any agent, even if the agent performed really poorly.

\subsection{FedAvg vs SumGrad}
FedAvg is according to the original paper supposed to be the superior actor, though there are some benefits to using the summed gradients.
The summed gradients, will lead to larger updates, so for environments where high rewards are less frequent, the summed gradients are more likely to allow the agent to more quickly change its actions towards something which is good.
The FedAvg leads to smaller updates, this means that the updates are more stable, and so for environments where the reward functions give a more regular reward it should learn more gradually than the summed gradients.

%Results


==> Sections/removed.tex <==
Abstract:
The R/L weighted methods replace standard practices for training multiple agents, such as summing or averaging the gradients. 
The core of our methods is the scaling of actors' gradients based on their reward (for R-Weighted) or their loss (for L-Weighted). 
During training, each agent operates with the same Neural Network parameters in differently initialized versions of the same environment, which gives different gradients from different actors. 
In essence, the R-Weighted and L-Weighted of each agent inform the other agents of its potential, which again reports which environment should be prioritized for learning. 
This distributed learning approach is possible because environments with higher rewards or losses may have more critical information than environments with lower rewards or losses. 

Results:
We have an effective implementation: the R-Weighted gradients.
R-Weighted gradient could get issues with the environments being the same, for example, a self-driving environment in which the road is the same.
If the environment is the same or very similar, then overfitting is very likely.
If the agent only has to turn left to get a high reward, it will always predict the left to be the best action.
An environment where the vehicle has to turn right would then get a low reward.
The L-Weighted gradient has issues with the fact that information from lower loss experiences may be more valuable, and if the low loss experiences are not trained on, then it will not learn what they are offering.
This means that both algorithms have a similar issue in that the weights used to scale the gradients cannot go too low; to counteract this, we included a hyperparameter that adds a number to the weight.
This weight is supposed to stabilize the gradients, though it also requires testing to find the correct value as it is a hyperparameter.
Testing the different values for this hyperparameter is to find the more stable, well-performing parameter.
When testing with a 1/16 value, we see that the performance is significantly worse than when testing with 1/8 in fig:\ref{fig:Softmax}; this makes sense as the training used eight agents; since eight agents were used for training, each agent at least has the same weight as it would during the Baseline-Avg, but could have a significantly higher value if its reward or loss is high, dependent on the algorithm used for training.

For our results, the graphs show us the general trend of these algorithms, with our R-Weighted and L-Weighted algorithms functioning similarly to that of the Baseline algorithms, as shown in fig:\ref{fig:PPOCartpole}, \ref{fig:PPOBipedal} and \ref{fig:PPOLunar}.
Our Actor-sum and Actor-avg algorithms do not perform well however, this could be due to the weights of each agent diverging from the starting point, thereby making the gradients of one agent useless to the other agents; we therefore only included it in fig:\ref{fig:PPOCartpole}. Another exciting find is that FedAvg does worse the more complex the environment is; this may be due to FedAvg being designed for supervised learning and being tested on MNIST and Cifar. The reason for this could be that the difference in the gradients is too large, leading to the gradients pulling in vastly different directions, or the worse gradients simply telling the algorithm what not to do when there is a lot more information in what gives a higher reward.

Results are pretty different when changing the size of the NN, though, as we can see the difference between each NN in fig:\ref{fig:PPOLunarEnd},\ref{fig:LunarMid},\ref{fig:LunarLarge}.
The performance differences for the size of the NN can have multiple reasons, one of which is overfitting.
When training while using the R-Weighted algorithm, there is a risk of it overfitting towards specific scenarios.
If the environment being trained in is simple, and NN is large, it is likely that having a large reward from one agent only happens a few times.
With the NN only optimizing a couple of high reward values, the training is more likely to skew towards overfitting those values initially and the model trying to generalize later.
When the model tries to generalize later, it will take longer to reach the optimal value, slowing compared to the baseline algorithms.

To more easily understand our results, we can show their average reward (avgRew) and the average reward from when the first algorithm moving average reached a threshold (avgEndRew), a reward of 100 for Lunarlander and 200 for BipedalWalker.
Using these scores, we can see which algorithm gets faster toward the optimum and which does best when converging.
If an algorithm gets up to a higher score faster, we see its avgRew being higher.
If an algorithm gets a higher avgEndRew, then the algorithm gets consistently high rewards in different randomly initiated environments after converging.

For the BipedalWalker environment, we see that the R-Weighted algorithm gets a higher avgRew and avgEndRew as shown in tab:\ref{tab:bipedal}.
While for the LunarLander environments, we find R-Weighted getting the highest rewards, shown in tab:\ref{tab:lunar}.

Looking at the episode number at which the algorithms reach the threshold of either 80, 400 or 200 depending on the gym environment, as shown in tab:\ref{tab:converge}, we find that for the CartPole environment, our R-Weighted underperforms the Baseline-sum, as shown in tab:\ref{tab:cartpole};
When we look at the BipedalWalker and LunarLander, however, we find that it is significantly better, especially in the more complex BipedalWalker environment.

The different environments have different complexities, as the LunarLander environment takes approximately 150 episodes for each agent to converge, and the BipedalWalker environment takes approximately 1200 episodes for each agent to converge.
This could imply that R-Weighted algorithm speeds up the learning and R-Weighted functions better for more complex environments.

To show the performance in a different light, we created a set of tables showing the results.
These tables include avgRew, meaning the total average reward for the environment, avgEndRew, which gives the average reward after the first algorithm reaches the threshold of the environment.
These thresholds are taken from the gym environment websites and shown in tab \ref{tab:converge} in parethesis.
All values are normalized on baseline-sum, and whenever its value is negative, we add the lowest reward to all algorithms before calculating the performance.
In tab \ref{tab:converge} we have some values, which are the length of the training with a + at the end; this is because they did not reach the threshold in time.
When listing the point at which the algorithm reached the threshold, we use the moving average with a value of 0.9 here.
